A Manually-Curated Dataset of Fixes to Vulnerabilities of Open-Source Software

Advancing our understanding of software vulnerabilities, automating their identification, the analysis of their impact, and ultimately their mitigation is necessary to enable the development of software that is more secure. While operating a vulnerability assessment tool that we developed and that is currently used by hundreds of development units at SAP, we manually collected and curated a dataset of vulnerabilities of open-source software and the commits fixing them. The data was obtained both from the National Vulnerability Database (NVD) and from project-specific Web resources that we monitor on a continuous basis. From that data, we extracted a dataset that maps 624 publicly disclosed vulnerabilities affecting 205 distinct open-source Java projects, used in SAP products or internal tools, onto the 1282 commits that fix them. Out of 624 vulnerabilities, 29 do not have a CVE identifier at all and 46, which do have a CVE identifier assigned by a numbering authority, are not available in the NVD yet. The dataset is released under an open-source license, together with supporting scripts that allow researchers to automatically retrieve the actual content of the commits from the corresponding repositories and to augment the attributes available for each instance. Also, these scripts allow to complement the dataset with additional instances that are not security fixes (which is useful, for example, in machine learning applications). Our dataset has been successfully used to train classifiers that could automatically identify security-relevant commits in code repositories. The release of this dataset and the supporting code as open-source will allow future research to be based on data of industrial relevance; also, it represents a concrete step towards making the maintenance of this dataset a shared effort involving open-source communities, academia, and the industry.

==> data/vuln_per_repo.tex <==
\footnotesize
\begin{tabular}{lc}
\toprule
                                          repo\_url &  distinct\_vuln \\
\midrule
                  https://github.com/apache/struts &             34 \\
              https://github.com/jenkinsci/jenkins &             19 \\
               https://github.com/cloudfoundry/uaa &             17 \\
                https://github.com/apache/activemq &             15 \\
             https://github.com/jenkinsci/jenkins/ &             14 \\
 https://github.com/spring-projects/spring-fram... &             14 \\
                   https://github.com/apache/camel &             11 \\
                     https://github.com/apache/cxf &             10 \\
          https://github.com/eclipse/jetty.project &             10 \\
             https://github.com/apache/lucene-solr &              8 \\
                  https://github.com/bcgit/bc-java &              7 \\
                 https://github.com/apache/hadoop/ &              7 \\
 https://github.com/spring-projects/spring-fram... &              7 \\
                 https://github.com/apache/tomcat/ &              7 \\
                 https://github.com/bcgit/bc-java/ &              6 \\
 https://github.com/spring-projects/spring-secu... &              6 \\
              https://github.com/cloudfoundry/uaa/ &              5 \\
    https://github.com/FasterXML/jackson-databind/ &              5 \\
               https://github.com/apache/cxf-fediz &              5 \\
                   https://github.com/apache/nifi/ &              5 \\
                   https://github.com/apache/tika/ &              5 \\
        % https://github.com/opennetworkinglab/onos/ &              4 \\
                  % https://github.com/rhuss/jolokia &              3 \\
          % https://github.com/elastic/elasticsearch &              3 \\
                % https://github.com/apache/syncope/ &              3 \\
             % https://github.com/vert-x3/vertx-web/ &              3 \\
              % https://github.com/apache/axis2-java &              3 \\
                    % https://github.com/netty/netty &              3 \\
               % https://github.com/x-stream/xstream &              3 \\
                   % https://github.com/apache/hive/ &              3 \\
     % https://github.com/FasterXML/jackson-databind &              3 \\
          % https://github.com/undertow-io/undertow/ &              3 \\
 % https://github.com/AsyncHttpClient/async-http-... &              3 \\
                    % https://github.com/tada/pljava &              2 \\
    % https://github.com/jenkinsci/subversion-plugin &              2 \\
         % https://github.com/javamelody/javamelody/ &              2 \\
            % https://github.com/apache/lucene-solr/ &              2 \\
              % https://github.com/pippo-java/pippo/ &              2 \\
                   % https://github.com/apache/karaf &              2 \\
 % https://github.com/spring-projects/spring-inte... &              2 \\
   % https://github.com/apache/httpcomponents-client &              2 \\
 % https://git.eclipse.org/r/hudson/org.eclipse.h... &              2 \\
         % https://github.com/OpenRefine/OpenRefine/ &              2 \\
               % https://github.com/square/retrofit/ &              2 \\
 % https://github.com/spring-projects/spring-data... &              2 \\
                    % https://github.com/apache/tika &              2 \\
          % https://github.com/javamelody/javamelody &              2 \\
             % https://github.com/keycloak/keycloak/ &              2 \\
                   % https://github.com/apache/sling &              2 \\
                  % https://github.com/apache/hadoop &              2 \\
    % https://github.com/spring-projects/spring-amqp &              2 \\
                 % https://github.com/apache/ignite/ &              2 \\
 % https://android.googlesource.com/platform/fram... &              2 \\
         % https://github.com/apache/cordova-android &              2 \\
                   % https://github.com/apache/hbase &              2 \\
              % https://github.com/keycloak/keycloak &              2 \\
                  % https://github.com/apache/storm/ &              2 \\
 % https://github.com/spring-projects/spring-webflow &              2 \\
 % https://github.com/FasterXML/jackson-dataforma... &              2 \\
       % https://github.com/kawasima/struts1-forever &              2 \\
         % https://github.com/SonarSource/sonarqube/ &              2 \\
        % https://github.com/apache/commons-compress &              2 \\
                   % https://github.com/apache/shiro &              2 \\
        % https://github.com/ESAPI/esapi-java-legacy &              2 \\
 % https://github.com/spring-projects/spring-secu... &              2 \\
                  % https://github.com/apache/camel/ &              2 \\
                % https://github.com/nahsra/antisamy &              2 \\
                  % https://github.com/apache/ambari &              2 \\
                  % https://github.com/apache/wicket &              2 \\
          % https://github.com/eclipse-ee4j/mojarra/ &              1 \\
              % https://github.com/apache/tapestry-5 &              1 \\
             % https://gerrit.ovirt.org/ovirt-engine &              1 \\
                 % https://github.com/junrar/junrar/ &              1 \\
             % https://github.com/fusesource/hawtjni &              1 \\
     % https://github.com/apache/directory-ldap-api/ &              1 \\
        % https://github.com/jenkinsci/junit-plugin/ &              1 \\
                  % https://github.com/apache/groovy &              1 \\
                 % https://github.com/apache/groovy/ &              1 \\
               % https://github.com/apache/activemq/ &              1 \\
 % https://github.com/pivotal-cf/spring-cloud-sso... &              1 \\
              % https://github.com/beobal/cassandra/ &              1 \\
  % https://github.com/codehaus-plexus/plexus-utils/ &              1 \\
                 % https://github.com/jkuhnert/ognl/ &              1 \\
 % https://android.googlesource.com/platform/fram... &              1 \\
         % https://github.com/zeroturnaround/zt-zip/ &              1 \\
    % https://github.com/jeremylong/DependencyCheck/ &              1 \\
 % https://github.com/jenkinsci/promoted-builds-p... &              1 \\
    % https://github.com/jenkinsci/ownership-plugin/ &              1 \\
         % https://github.com/infinispan/infinispan/ &              1 \\
              % https://github.com/google/conscrypt/ &              1 \\
                 % https://github.com/apache/syncope &              1 \\
 % https://github.com/jenkinsci/google-play-andro... &              1 \\
                 % https://github.com/apache/cayenne &              1 \\
                   % https://github.com/apache/geode &              1 \\
    % https://github.com/jenkinsci/saltstack-plugin/ &              1 \\
 % https://android.googlesource.com/platform//ext... &              1 \\
          % https://github.com/blynkkk/blynk-server/ &              1 \\
    % https://github.com/jenkinsci/ssh-agent-plugin/ &              1 \\
 % https://github.com/spring-projects/spring-secu... &              1 \\
             % https://github.com/apache/uima-uimaj/ &              1 \\
                  % https://github.com/apache/hbase/ &              1 \\
            % https://github.com/orbeon/orbeon-forms &              1 \\
        % https://github.com/igniterealtime/Openfire &              1 \\
   % https://github.com/jenkinsci/checkstyle-plugin/ &              1 \\
  % https://github.com/spring-projects/spring-social &              1 \\
 % https://github.com/codehaus-plexus/plexus-arch... &              1 \\
                  % https://github.com/apache/ranger &              1 \\
     % https://github.com/lingochamp/FileDownloader/ &              1 \\
   % https://github.com/rabbitmq/rabbitmq-jms-client &              1 \\
                % https://github.com/apache/zeppelin &              1 \\
         % https://github.com/apache/brooklyn-server &              1 \\
 % https://github.com/spring-projects/spring-inte... &              1 \\
 % https://github.com/apache/sling-org-apache-sli... &              1 \\
          % https://github.com/primefaces/primefaces &              1 \\
                   % https://github.com/itext/itext7 &              1 \\
        % https://github.com/apache/activemq-artemis &              1 \\
                   % https://github.com/apache/tomee &              1 \\
                    % https://github.com/google/gson &              1 \\
           % https://github.com/jenkinsci/pmd-plugin &              1 \\
                 % https://github.com/apache/struts/ &              1 \\
              % https://github.com/droolsjbpm/drools &              1 \\
                  % https://github.com/google/guava/ &              1 \\
   % https://github.com/jenkinsci/monitoring-plugin/ &              1 \\
  % https://github.com/micromata/projectforge-webapp &              1 \\
     % https://github.com/orientechnologies/orientdb &              1 \\
               % https://github.com/apache/cassandra &              1 \\
            % https://github.com/candlepin/candlepin &              1 \\
                 % https://github.com/djmdjm/jBCrypt &              1 \\
         % https://github.com/eclipse/jetty.project/ &              1 \\
          % https://github.com/jenkinsci/ccm-plugin/ &              1 \\
                   % https://github.com/umlet/umlet/ &              1 \\
                  % https://github.com/apache/oozie/ &              1 \\
              % https://github.com/OpenTSDB/opentsdb &              1 \\
                 % https://github.com/apache/thrift/ &              1 \\
                   % https://github.com/neo4j/neo4j/ &              1 \\
          % https://github.com/jenkinsci/ec2-plugin/ &              1 \\
 % https://github.com/spring-projects/spring-secu... &              1 \\
     % https://github.com/jenkinsci/mercurial-plugin &              1 \\
                  % https://github.com/apache/batik/ &              1 \\
                     % https://github.com/jhy/jsoup/ &              1 \\
                    % https://github.com/dom4j/dom4j &              1 \\
        % https://github.com/jenkinsci/mailer-plugin &              1 \\
              % https://github.com/apache/xerces2-j/ &              1 \\
                 % https://github.com/itext/itextpdf &              1 \\
         % https://github.com/apereo/java-cas-client &              1 \\
 % https://github.com/jenkinsci/android-lint-plugin/ &              1 \\
 % https://github.com/jenkinsci/depgraph-view-plu... &              1 \\
    % https://github.com/swagger-api/swagger-codegen &              1 \\
                  % https://github.com/square/okhttp &              1 \\
          % https://github.com/apache/portals-pluto/ &              1 \\
                  % https://github.com/apache/geode/ &              1 \\
          % https://github.com/apache/logging-log4j2 &              1 \\
             % https://github.com/SvenEwald/xmlbeam/ &              1 \\
               % https://github.com/seam2/jboss-seam &              1 \\
      % https://github.com/jenkinsci/ansible-plugin/ &              1 \\
 % https://github.com/cloudfoundry-incubator/credhub &              1 \\
                  % https://github.com/apache/karaf/ &              1 \\
          % https://github.com/eclipse-vertx/vert.x/ &              1 \\
     % https://github.com/jenkinsci/coverity-plugin/ &              1 \\
 % https://github.com/hibernate/hibernate-validator/ &              1 \\
           % https://github.com/jenkinsci/git-plugin &              1 \\
                    % https://github.com/apache/cxf/ &              1 \\
 % https://github.com/deeplearning4j/deeplearning4j/ &              1 \\
                  % https://github.com/looly/hutool/ &              1 \\
         % https://github.com/BigBadaboom/androidsvg &              1 \\
                 % https://github.com/facebook/buck/ &              1 \\
           % https://github.com/inversoft/prime-jwt/ &              1 \\
                  % https://github.com/apache/spark/ &              1 \\
                  % https://github.com/apache/kafka/ &              1 \\
  % https://github.com/hibernate/hibernate-validator &              1 \\
        % https://github.com/sebfz1/wicket-jquery-ui &              1 \\
            % https://github.com/jythontools/jython/ &              1 \\
                    % https://github.com/apache/poi/ &              1 \\
 % https://github.com/jenkinsci/gerrit-trigger-pl... &              1 \\
 % https://github.com/apache/cordova-plugin-file-... &              1 \\
          % https://github.com/wildfly/wildfly-core/ &              1 \\
    % https://github.com/jenkinsci/email-ext-plugin/ &              1 \\
               % https://github.com/letonez/libpam4j &              1 \\
              % https://github.com/apache/cxf-fediz/ &              1 \\
   % https://github.com/spring-projects/spring-amqp/ &              1 \\
                    % https://github.com/apache/nifi &              1 \\
           % https://github.com/apache/qpid-broker-j &              1 \\
                 % https://github.com/qos-ch/logback &              1 \\
 % https://github.com/restlet/restlet-framework-java &              1 \\
 % https://github.com/spring-projects/spring-data... &              1 \\
       % https://github.com/sebfz1/wicket-jquery-ui/ &              1 \\
                 % https://github.com/eclipse/vert.x &              1 \\
                  % https://github.com/pslegr/core-1 &              1 \\
         % https://github.com/OPCFoundation/UA-Java/ &              1 \\
           % https://github.com/pingidentity/ldapsdk &              1 \\
     % https://github.com/jenkinsci/favorite-plugin/ &              1 \\
          % https://github.com/apache/qpid-proton-j/ &              1 \\
                    % https://github.com/apache/hive &              1 \\
                      % https://github.com/weld/core &              1 \\
                 % https://github.com/eclipse/rdf4j/ &              1 \\
                 % https://github.com/hawtio/hawtio/ &              1 \\
                  % https://github.com/apache/derby/ &              1 \\
                     % https://github.com/apache/poi &              1 \\
            % https://github.com/inversoft/prime-jwt &              1 \\
          % https://github.com/apache/qpid-broker-j/ &              1 \\
             % https://github.com/jboss-fuse/jasypt/ &              1 \\
                   % https://github.com/apache/atlas &              1 \\
   % https://github.com/jenkinsci/kubernetes-plugin/ &              1 \\
      % https://github.com/jenkinsci/groovy-sandbox/ &              1 \\
 % https://android.googlesource.com/platform/pack... &              1 \\
 % https://github.com/restlet/restlet-framework-j... &              1 \\
            % https://github.com/beanshell/beanshell &              1 \\
 % https://github.com/spring-projects/spring-data... &              1 \\
           % https://github.com/Wechat-Group/WxJava/ &              1 \\
               % https://github.com/wildfly/wildfly/ &              1 \\
               % https://github.com/belaban/JGroups/ &              1 \\
       % https://github.com/apache/commons-compress/ &              1 \\
         % https://github.com/apache/activemq-apollo &              1 \\
                % https://github.com/narkisr/nmap4j/ &              1 \\
             % https://github.com/apache/axis1-java/ &              1 \\
 % https://github.com/jenkinsci/tikal-multijob-pl... &              1 \\
    % https://github.com/spring-projects/spring-ldap &              1 \\
  % http://git.bouncycastle.org/repositories/bc-java &              1 \\
         % https://github.com/kiegroup/jbpm-designer &              1 \\
              % https://github.com/ronsigal/Resteasy &              1 \\
 % https://github.com/jenkinsci/pipeline-build-st... &              1 \\
                 % https://github.com/apache/pdfbox/ &              1 \\
           % https://github.com/undertow-io/undertow &              1 \\
 % https://github.com/jenkinsci/build-publisher-p... &              1 \\
      % https://github.com/apache/commons-fileupload &              1 \\
                  % https://github.com/pgjdbc/pgjdbc &              1 \\
   % https://github.com/jenkinsci/git-client-plugin/ &              1 \\
\bottomrule
\end{tabular}


==> macros.tex <==
%%%%%%%%%%
%% NOTE: THIS IS NOT INCLUDED ANY LONGER, PLEASE SEE data/data_from_notebook.tex
%%%%%%%%%%

\newcommand{\VULNBEFORE}{509\xspace}
\newcommand{\VULNAFTER}{484\xspace}
\newcommand{\VULNAFTERNOCVE}{27\xspace}
\newcommand{\VULNAFTERNONVD}{42\xspace}
\newcommand{\REPOBEFORE}{229\xspace}
\newcommand{\REPOAFTER}{227\xspace}
\newcommand{\COMMITBEFORE}{1437\xspace}
\newcommand{\COMMITAFTER}{634\xspace}
\newcommand{\DATASETSIZEALL}{2715???\xspace}
\newcommand{\DATASETSIZENEG}{2259???\xspace}
\newcommand{\DATASETSIZEPOS}{456\xspace}


==> related_work.tex <==
% \section{Related Work}
% \label{sec:relwork}
% Vulnerability datasets like the one we used are a precious (and scarce) resource. Perl et al.~\cite{Perl:2015:VFP:2810103.2813604},
% as part of their work on finding \emph{Vulnerability Contributing Commits} (VCC),
% have produced what they claim to be the largest (public) database of mappings between CVEs affecting OSS and the
% commits that \emph{introduced} the vulnerability. Their methodology, although automated, only considers CVEs that include an explicit reference to the corresponding commit(s); in our experience, these references are rather rare and often inaccurate. The dataset of~\cite{Perl:2015:VFP:2810103.2813604} includes 640 commits, corresponding to 718 CVEs, affecting 66 C/C++ projects.

% Commercial vendors such as SourceClear (\url{http://sourceclear.com}) and Snyk (\url{http://snyk.io/vuln}) provide vulnerability data through their Web pages; Snyk also publishes monthly dumps of their databases on GitHub.
% These resources could be used to replicate our study.


==> tables/joint.tex <==
\begin{tabular}{ccccc}
\toprule
 pos\_weight &  accuracy &  f1-score &  precision &  recall \\
\midrule
        0.05 &      0.83 &      0.10 &       0.10 &    0.05 \\
       0.10 &      0.84 &      0.13 &       0.47 &    0.07 \\
        0.15 &      0.85 &      0.25 &       0.91 &    0.15 \\
       0.20 &      0.86 &      0.33 &       0.94 &    0.20 \\
        0.25 &      0.87 &      0.43 &       0.85 &    0.28 \\
       0.30 &      0.88 &      0.48 &       0.85 &    0.34 \\
        0.35 &      0.89 &      0.53 &       0.83 &    0.40 \\
       0.40 &      0.89 &      0.57 &       0.78 &    0.46 \\
        0.45 &      0.89 &      0.58 &       0.74 &    0.49 \\
       0.50 &      0.89 &      0.61 &       0.73 &    0.53 \\
        0.55 &      0.88 &      0.63 &       0.68 &    0.59 \\
       0.60 &      0.88 &      0.63 &       0.65 &    0.63 \\
        0.65 &      0.87 &      0.64 &       0.61 &    0.68 \\
       0.70 &      0.86 &      0.63 &       0.57 &    0.71 \\
        0.75 &      0.85 &      0.64 &       0.55 &    0.79 \\
       0.80 &      0.83 &      0.61 &       0.49 &    0.82 \\
        0.85 &      0.78 &      0.56 &       0.42 &    0.84 \\
       0.90 &      0.69 &      0.50 &       0.34 &    0.91 \\
       0.95 &      0.47 &      0.38 &       0.24 &    0.99 \\
\bottomrule
\end{tabular}


==> tables/msg.tex <==
\begin{tabular}{ccccc}
\toprule
 pos\_weight &  accuracy &  f1-score &  precision &  recall \\
\midrule
        0.05 &      0.83 &      0.08 &       0.05 &    0.04 \\
       0.10 &      0.84 &      0.09 &       0.55 &    0.05 \\
        0.15 &      0.85 &      0.20 &       0.92 &    0.11 \\
       0.20 &      0.85 &      0.24 &       0.95 &    0.15 \\
        0.25 &      0.86 &      0.31 &       0.90 &    0.19 \\
       0.30 &      0.86 &      0.33 &       0.86 &    0.21 \\
        0.35 &      0.87 &      0.38 &       0.83 &    0.25 \\
       0.40 &      0.87 &      0.43 &       0.80 &    0.30 \\
        0.45 &      0.87 &      0.45 &       0.78 &    0.32 \\
       0.50 &      0.87 &      0.46 &       0.74 &    0.34 \\
        0.55 &      0.87 &      0.49 &       0.71 &    0.38 \\
       0.60 &      0.87 &      0.49 &       0.69 &    0.38 \\
        0.65 &      0.86 &      0.50 &       0.64 &    0.42 \\
       0.70 &      0.86 &      0.53 &       0.64 &    0.47 \\
        0.75 &      0.85 &      0.53 &       0.58 &    0.50 \\
       0.80 &      0.85 &      0.54 &       0.55 &    0.55 \\
        0.85 &      0.83 &      0.54 &       0.49 &    0.62 \\
       0.90 &      0.78 &      0.52 &       0.42 &    0.72 \\
       0.95 &      0.59 &      0.42 &       0.28 &    0.89 \\
\bottomrule
\end{tabular}


==> tables/patch.tex <==
\begin{tabular}{ccccc}
\toprule
 pos\_weight &  accuracy &  f1-score &  precision &  recall \\
\midrule
        0.05 &      0.83 &         - &       0.00 &       - \\
       0.10 &      0.83 &      0.08 &       0.12 &    0.04 \\
        0.15 &      0.84 &      0.13 &       0.76 &    0.07 \\
       0.20 &      0.85 &      0.17 &       0.79 &    0.10 \\
        0.25 &      0.85 &      0.25 &       0.93 &    0.15 \\
       0.30 &      0.86 &      0.32 &       0.86 &    0.21 \\
        0.35 &      0.87 &      0.39 &       0.86 &    0.26 \\
       0.40 &      0.87 &      0.43 &       0.81 &    0.29 \\
        0.45 &      0.88 &      0.48 &       0.79 &    0.35 \\
       0.50 &      0.87 &      0.49 &       0.73 &    0.38 \\
        0.55 &      0.88 &      0.56 &       0.75 &    0.45 \\
       0.60 &      0.88 &      0.56 &       0.71 &    0.47 \\
        0.65 &      0.88 &      0.60 &       0.71 &    0.53 \\
       0.70 &      0.88 &      0.60 &       0.67 &    0.56 \\
        0.75 &      0.87 &      0.62 &       0.63 &    0.63 \\
       0.80 &      0.86 &      0.61 &       0.57 &    0.68 \\
        0.85 &      0.84 &      0.59 &       0.51 &    0.71 \\
       0.90 &      0.79 &      0.56 &       0.43 &    0.79 \\
       0.95 &      0.64 &      0.47 &       0.31 &    0.93 \\
\bottomrule
\end{tabular}

